SaLoBa: Maximizing Data Locality and Workload Balance for Fast Sequence Alignment on GPUs

Sequence alignment forms an important backbone in many sequencing applications. A commonly used strategy for sequence alignment is an approximate string matching with a two-dimensional dynamic programming approach. Although some prior work has been conducted on GPU acceleration of a sequence alignment, we identify several shortcomings that limit exploiting the full computational capability of modern GPUs. This paper presents SaLoBa, a GPU-accelerated sequence alignment library focused on seed extension. Based on the analysis of previous work with real-world sequencing data, we propose techniques to exploit the data locality and improve workload balancing. The experimental results reveal that SaLoBa significantly improves the seed extension kernel compared to state-of-the-art GPU-based methods.

==> index.tex <==
%\pagenumbering{roman}
%\thispagestyle{plain}
\begin{titlepage}
\thispagestyle{empty}
\pagenumbering{gobble}
%\pagestyle{plain}
\begin{figure*}

\large

     \fbox{\begin{minipage}{0.95\textwidth}We sincerely thank the reviewers for their time and valued comments. We have faithfully revised our paper and addressed each reviewers' comments below with much appreciation. All the revised texts are written in {\color{olivegreen}green color} with magenta markers {\color{magenta}{R1-R8}} around them. Please find the index below with \underline{hyperlinks} to them. 
     
     \begin{itemize}
     \small
         \item New table: \tabref{baselines}
         \item Additional experimental data:   \figref{histo250}, \figref{kernelall}, \figref{realkernel}
         
              \end{itemize}
     \end{minipage}} 

\vspace{5mm}

\underline{\huge\textbf{\textsf{Index}}}
\vspace{3mm}
%\small
\begin{enumerate}

\item \textbf {Comparison with more state-of-the-art implementations (reviewer 1/4):} 
\begin{itemize}
\item \revref{R1a} (p.6, left)
\item \revref{R1b} (p.7, left)
\item \revref{R1c} (p.9, left)
\item \tabref{baselines} 
\item \figref{kernelall}
\item \figref{realkernel}
\end{itemize}

\item \textbf {Explain losses and gains against short reads and long reads (reviewer 4):} 
\begin{itemize}
\item \figref{histo250}
\item \revref{R2a} (p.3, right)
\item \revref{R2b} (p.3, left)
\item \revref{R2c} (p.8, left)
\end{itemize}


\item \textbf {Provide dataset details (reviewer 3):} 
\begin{itemize}
\item \revref{R3} (p.8, right)
\item \revref{R2b} (p.3, left)
\end{itemize}


\item \textbf {Confusion on the need for inter-warp synchronization in \figref{vwc} (reviewer 3):} 
\begin{itemize}
\item \figref{vwc}
\item \revref{R4} (p.6, right)
\end{itemize}


\item{\textbf{Clarification of the 100x runtime balance (reviewer 3):}}
\begin{itemize}
\item \revref{R2a} (p.3, right)
\end{itemize}




\item \textbf {More thorough literature survey (reviewer 4):} 
\begin{itemize}
\item \revref{R6a} (p.2, right)
\item \revref{R6b} (p.9, left)
\end{itemize}

\item \textbf {Outdated statement regarding independent thread scheduling (reviewer 2):} 
\begin{itemize}
\item \revref{R7} (p.4, left)
\end{itemize}



\item \textbf {Better explain \figref{shm} about the relation between threads and blocks (reviewer 3):} 
\begin{itemize}
\item \figref{shm}
\item \revref{R8} (p.5, left)
\end{itemize}


\item \textbf {Figure placements (reviewer 3):} 
\begin{itemize}
\item \figref{parallel}
\item \figref{shm}
\item \figref{vwc}
\end{itemize}

\item \textbf {Grammar issues and typos (reviewer 1/2/3).} 









\end{enumerate}
\end{figure*}

\end{titlepage}

==> old_HW_related.tex <==

\rev{
\subsection{FPGA/ASIC Acceleration}

Due to its flexibility, FPGAs often become the target platform for emerging applications requiring fast deployment time. 
\cite{zhang2007implementation} provided  a detailed implementation of the Smith--Waterman algorithm on an Altera FPGA, followed by a few other studies using banded algorithms~\cite{chen2013hardware, blastp} or flexible systolic arrays~\cite{houtgast2015fpga,ahmed2015heterogeneous}. 
Moreover, DRAGEN~\cite{dragen} is an FPGA-based platform from Illumina that provides speedup by implementing the full end-to-end analysis into an FPGA.
These approaches adopt similar intra-query parallelization strategies with the GPU-based ones.
However, FPGAs are still hard to find from the market as accelerators.



%Aside from the extensions, some work has targeted seeding~\cite{cong2018smem++, subramaniyan2021accelerated}, or INDEL realignments~\cite{wu2019fpga}. 
%Further, Genesis~\cite{ham2020genesis} employed an FPGA as a service model and provided a framework for using extended SQL for the genomics pipeline.


%As interest in the genomics pipeline has increased, more
Some researchers have considered dedicated ASIC accelerators~\cite{primer}. 
Compared to FPGAs, ASICs provide better performance and energy efficiency at the expense of flexibility.  Darwin~\cite{turakhia2018darwin,turakhia2019darwin} is an accelerator that speeds up the whole genome sequencing through the co design of both the software and hardware, powered by gapped filtering. 
GenAx~\cite{fujiki2018genax} is an automata-based accelerator for both seeding and extension that supports configurable scoring and traceback functionality. 
Moreover, GenASM~\cite{genasm} is an accelerator framework for bitvector-based algorithms. 

\begin{comment}
The EXMA~\cite{jiang2021exma} accelerator designs a row-buffer friendly algorithm for the FM  index to build a dedicated accelerator. 
Further, SeedEx~\cite{fujiki2020seedex} is an extension accelerator that uses a banded algorithm. By opportunistically using a narrower band than required and providing a function that checks the optimality, it greatly reduces the width of the band used for extension algorithms.

\end{comment}
 


Although these researchers have claimed that they can achieve multi fold speedup, sometimes by a few hundred, ASICs fall into a solution that requires at least a few years to reach the market. 
Compared to them, GPU-based alignment software could be a quick solution easily adopted by any system that has GPUs attached.


}


==> thx.tex <==


%\Large
\underline{\Large\textbf{\textsf{Responses to Reviewers’ Comments}}}

% \hl{checklist}
% index page/position
% Check positions of figures
% remove highlights and comments jl, nh
% page number format

\vspace {5mm}
We sincerely thank the reviewers for their time and valued comments. 
We have faithfully revised our paper and addressed each reviewers' comments below with much appreciation. 
To highlight the major modifications, we have added more experimental comparisons to the prior work and did a more thorough literature survey.
Also, we have added various clarifications according to the comments and questions from the reviewers.
All the revised texts are written in {\color{olivegreen}green color} with magenta markers {\color{magenta}{R1-R8}} around them.  


     \begin{enumerate}
     
     
     %other kernels
         \item {\textbf{Comparison with more state-of-the-art implementations.} }
         
         \emph{\textbf{- ``As this is a performance-critical kernel in an important problem, there should be multiple implementations that could be described and evaluated'' (Reviewer 1).}}
         
         \emph{\textbf{- ``There isn't a thorough comparison to other state-of-the-art GPU-accelerated sequence aligners'' (Reviewer 4).} }
         
         \vspace{2mm} Thank you so much for the review. We have added five more seed extension GPU kernels listed in \tabref{baselines} into comparison. SOAP3-dp~\cite{soap3dp}, CUSHAW2-GPU~\cite{cushaw2gpu}, and NVBIO~\cite{nvbio} are kernels with inter-query parallelism and SW\#~\cite{korpar2013sw} and ADEPT~\cite{adept} are kernels for intra-query parallelism. 
         Some previous work was excluded from comparison for reasons such as using a totally different algorithm (GPU-RMAP) or seed extension performed on a CPU (cuBLASTP).
         
         \vspace{2mm}We faithfully optimized each kernel to our best. Most importantly, the current state-of-the-art kernel GASAL2~\cite{gasal2} is known to gain its performance from on-GPU bit packing. 
         We combined all the other kernels with the on-GPU packing from GASAL2 to ensure that we give reasonable and fair advantage to the baselines. 
         
         \vspace{2mm}One surprising result was that when combined with the on-GPU bit packing, NVBIO and CUSHAW2-GPU were found to perform comparably, and sometimes better than GASAL2. 
         However, \aligner still showed superior performance to all other kernels, as displayed in \figref{kernelall} and \figref{realkernel}.
         
         \vspace{2mm} Please find the associated revisions around markers \revref{R1a}, \revref{R1b}, and \revref{R1c}.
         
         \vspace{5mm}
                  
         
         
     %long sequence
         \item{\textbf{Explain differences between performance on different GPUs and for
different sequence lengths with the emphasis on what is gained for long
lengths and lost for short lengths. }}
          
         \emph{\textbf{- ``While a core motivation of this work is to efficiently handle relatively long sequence reads, the maximum performance gain was achieved on smaller read sizes (64bp)'' (Reviewer 4).}}
         
         \vspace{2mm} Thank you for the suggestion. By analyzing the results, we find that the counterintuitive gain at 64 bp is due to GASAL2's memory initialization cost, rather than \aligner being faster with 64 bp, as shown in \figref{kernelall}. GASAL2 has a large fixed cost for memory initialization which does not get amortized well with short sequences. 
         An additional comparison with NVBIO reveals that the gain from \aligner is observed only for sequences equal or longer than 128 bp.
         
         \vspace{2mm} To further study the impact of \aligner on long sequence reads, we added a real-world dataset from a 3rd generation sequencer, whose read lengths reach up to thousands. 
         As expected, the results in \figref{realkernel} (b) demonstrate that \aligner achieves even more speedup on the long read dataset than on short reads.         
         
          \vspace{2mm} Please find the associated revisions around markers \revref{R2a}, \revref{R2b}, and \revref{R2c}.
         
         
         
         \vspace{5mm}
    
    % dataset  
          \item{\textbf{Provide dataset details.}}
          
          \emph{\textbf{- ``What are the sizes of the datasets used in the evaluation?'' (Reviewer 3)}}
          
         \vspace{2mm} Thanks for the suggestion, and please find the added explanations around marker \revref{R3}. In sequence alignment, there are two input sequences: reference and query. For the reference, we use the DNA sequence of the entire human genome available from the human genome project. The sequence is in total 3.1 Gbp (base pair). 
         
         \vspace{2mm} The \textbf{dataset A} (SRR835433) is from a 2nd generation sequencer Illumina MiSeq and represents short reads 
        where each sequence has a length of 250 bp. 
        The dataset comprises 8.3 M sequences which are randomly read genome parts from a human. 
        Each sequence is read twice, resulting in the total number of base pairs to be 250$\times$8.3M$\times$2=4.1 Gbp.
        
        
         \vspace{2mm} The \textbf{dataset B} (SRP091981) is from a 3rd generation sequencer PacBio RS and represents long reads.
        It also contains randomly read genome parts from a human where there are 82K sequences with variable lengths that averages around 2,000 bp to a total of 182.4 Mbp.
                
         \vspace{2mm} The two sequences are processed by BWA-MEM to obtain seeds that can be extended with \aligner. \figref{histo250} around marker \revref{R2b} has been updated to contain the distribution of the lengths of both datasets.
%


         
         \vspace{5mm}
    
    % sync    
         \item \textbf {Confusion on the need for inter-warp synchronization in \figref{vwc}.} 
                   
          \emph{\textbf{- ``The necessary synchronization between warps working on neighboring chunks is unclear'' (Reviewer 3)}}
         
         \vspace{2mm} We apologize for the confusion. From the reviewer's comment, we noticed that the original \figref{vwc} could mislead the readers.
         For example, the original figure could be understood as if inter-warp synchronization is required (e.g., multiple warps cooperatively process a single query through inter-warp synchronization as the reviewer previously interpreted).
         
         \vspace{2mm}
         
         In fact, \aligner{} does not require inter-warp synchronization by assigning only one warp (or subwarp) to a single query.
         As a result, ensuring that the intra-warp threads move on together to the next chunk suffices. 
         
         \vspace{2mm} We have modified \figref{vwc} accordingly to avoid the confusion. Please find it around marker \revref{R4}.
         
         
         

         
         \vspace{5mm}
    % dataset  
          \item{\textbf{Clarification of the 100x runtime balance.}}
          
          \emph{\textbf{- ``The most I can see in Figure is a difference of 5 or 6 (between 125bp and 250 bp). How do you get to 100x? (Reviewer 3)}}
          
         \vspace{2mm} We apologize for the confusion. The computation complexity of the seed extension given by Smith--Waterman algorithm is the product of the two input sequence lengths. 
         From the \figref{histo250} for short reads, the maximum difference found from query and reference are both around 10x (25bp - 250bp for query and 50bp - 500bp for reference). Considering this, the worst case imbalance could be a multiple of the two differences (i.e., 10x10=100). However, we agree that it could be misleading as such a case would be very rare. We modified the explanation around \revref{R2a} accordingly.
          
         \vspace{5mm}
                  
         
     %long sequence
              \item{\textbf{More thorough literature survey.}}
              
              \emph{\textbf{- ``A more extensive literature search should have been done to see what other tools have been proposed to map onto a GPU'' (Reviewer 4).}}
              
                 \vspace{2mm} Thanks for the review. As suggested by the reviewer, we have re-written most of the related work section (\revref{R6b}) and focused more on GPU acceleration by cutting out some hardware-only approaches. Furthermore, we modified the background section to include more general schemes for GPU-based seed extension (\revref{R6a}).
                  

         \vspace{5mm}
            
    % ITS
         \item{\textbf{Outdated statement regarding independent thread scheduling.}}
              
         \emph{\textbf{- ``There is one out-of-date statement about thread scheduling on NVIDIA GPUs.'' (Reviewer 2).}}

         \vspace{2mm}         
         Thanks for the comment. We have revised the description around marker \revref{R7} to reflect the changes associated with independent thread scheduling.     
         

         
         
         
         
         \vspace{5mm}
    
    % figure 4        
          \item{\textbf{Better explain \figref{shm} about the relation between threads and blocks.}}
              
         \emph{\textbf{- ``In Figure 4b, it is not immediately clear what relation between the threads t* and the Blocks* is'' (Reviewer 3)}}
         
         \vspace{2mm} Thanks for the comment and we apologize for the confusion. In \figref{shm}, each small rectangle represents 8×1 cells stored for dependency. When occupied by colored rectangles denoted `t\#', it is being accessed by the thread \#. When denoted `block \#', it is the value from the block id \# and is ready to be spilled to the global memory. Please find the explanation in the caption of \figref{shm} around marker \revref{R8}.
         
         
         
         
         \vspace{5mm}
    
    % figure placements      
          \item{\textbf{Figure placements.}}
             
         \emph{\textbf{- ``The figure placement could be improved: having large explanatory figures (3, 4, 5) closer to where they are described in the text'' (Reviewer 3)}} 
         
         \vspace{2mm} Thanks for the comment. We have adjusted the text and figure locations, and now the figures are closer to where they are mentioned.
         
         
         \vspace{5mm}
    
    % grammar    
          \item{\textbf{Grammar issues and typos.}}
          
          \emph{\textbf{- ``Address language issues'' (Reviewer 1)}}
          
          \emph{\textbf{- ``I notice a few minor grammar issues'' (Reviewer 2)}}
          
          \emph{\textbf{- ``It would certainly benefit from a thorough proof-reading pass to eliminate grammatical mistakes and typos'' (Reviewer 3)}}
          
         \vspace{2mm} Thank you so much for the kind comments. We have done several rounds of proofreading and grammar checks. We believe it is now in a much better shape.
          
     \end{enumerate} 
%\pagebreak


\newpage


%\large



